Zero-shot Approach to Overcome Perturbation Sensitivity of Prompts

Recent studies have demonstrated that natural-language prompts can help to leverage the knowledge learned by pre-trained language models for the binary sentence-level sentiment classification task. Specifically, these methods utilize few-shot learning settings to fine-tune the sentiment classification model using manual or automatically generated prompts. However, the performance of these methods is sensitive to the perturbations of the utilized prompts. Furthermore, these methods depend on a few labeled instances for automatic prompt generation and prompt ranking. This study aims to find high-quality prompts for the given task in a zero-shot setting. Given a base prompt, our proposed approach automatically generates multiple prompts similar to the base prompt employing positional, reasoning, and paraphrasing techniques and then ranks the prompts using a novel metric. We empirically demonstrate that the top-ranked prompts are high-quality and significantly outperform the base prompt and the prompts generated using few-shot learning for the binary sentence-level sentiment classification task.

==> backup.tex <==
% \subsection{Automatic Prompt Generation}
% \label{second}
% Given the base prompt ($B_p$), we generate multiple prompts using position, reasoning, and paraphrasing techniques. The positioning technique arranges the prompt either before or after the sentence. The reasoning technique combines the sentence and the prompt using words like \textit{because, so}, etc. If the prompt is before the sentence, the word \textit{because} is used, and if the prompt is after the sentence, the word \textit{so} is used to combine the sentence and the prompt. The words \textit{because, so} enable the model to relate the label with the context of the sentence. The paraphrasing technique swaps the words of the base prompt with similar words to obtain new prompts. The pre-trained masked language model $\mathcal{L}$ is used to obtain similar words. First, a sentence is sampled from the weakly labeled dataset $\mathcal{D'}$ and combined with the base template using \textit{because or so} to obtain a sample instance. For example, if the sampled sentence is, \textit{burger was great} and the corresponding weak label is \textit{positive}. Using the base prompt in Figure \ref{fig:input}, the sample instance is \textit{"the sentence was positive because burger was great"}. Next, we mask the tokens of the base prompt one after another and get top $K$ ranked predictions of the model $\mathcal{L}$ as similar word candidates. The candidates whose pos-tag matches the masked token's pos-tag are considered similar words to the masked token. For example, if we mask the token \textit{the}, the updated sample instance is \textit{"[MASK] sentence was positive because burger was great"} and some of the similar words are \textit{my, a, this}. The similar words of corresponding base prompt tokens are combined to obtain new prompts. The position and reasoning techniques are applied to the new prompts to obtain automatically generated prompts. The hyperparameter $K$ can be increased to obtain more prompts.

% \subsection{Weak Labeled Dataset}
% Given an input mapping $\mathcal{M}:\mathcal{Y}\rightarrow\mathcal{V}$ as shown in Figure \ref{fig:input}, we first obtain the mapping tokens ($\in \mathcal{V}$) of the labels ($\in \mathcal{Y}$). For example, the mapping tokens and corresponding labels for the input mapping in Figure \ref{fig:input} are \textit{\{great, terrible\}} and \textit{\{positive, negative\}}, respectively. Then, WordNet is used to obtain synonyms for each mapping token. Next, we search through the corpus $\mathcal{D}$ to find sentences that contain mapping tokens; if found, we add the sentence to the weakly labeled dataset $\mathcal{D'}$ along with the label corresponding to the mapping token as the label. We also replace the mapping token with the other mapping token in the sentence to obtain a new sentence and label it with the corresponding label of the other mapping token. We similarly search corpus $\mathcal{D}$ to find sentences that contain synonyms of the mapping tokens and add them to $\mathcal{D'}$ along with the label. We utilize the weakly labeled dataset $\mathcal{D'}$ in the second and third steps discussed in Section \ref{second} and \ref{third}.

% \subsection{Prompt Ranking}
% \label{third}
% Given the input mapping $\mathcal{M}:\mathcal{Y}\rightarrow\mathcal{V}$ from the task label space to individual words in the vocabulary $\mathcal{V}$ of the model $\mathcal{L}$. The prompt $P$ generated automatically is evaluated as follows: for each sentence $s_{in}$ in the weakly labeled dataset $\mathcal{D'}$, let the manipulation after applying the prompt $P$ be $s_{P} = P(s_{in})$ which contains exactly one masked token at the position of the label. For example, \textit{"the sentence was [MASK] because burger was great"}. $s_{P}$ is given as the input to the masked language model $\mathcal{L}$. Therefore, the task is MLM, and the probability of predicting class $y \in \mathcal{Y}$ is modeled as:
% \begin{align*}
%     p(y|s_{in}) = p([MASK] = \mathcal{M}(y) | s_{P}) \\ = \frac{exp(w_{\mathcal{M}(y)}.h_{[MASK]})}{\sum_{y' \in \mathcal{Y}} exp(w_{\mathcal{M}(y')}.h_{[MASK]})},
% \end{align*}

% where $h_{[MASK]}$ is the hidden vector of $[MASK]$ and $w_v$ denotes the pre-softmax vector corresponding to $v \in \mathcal{Y}$. Each prompt $P$ generated automatically is evaluated on the weak labeled dataset $\mathcal{D'}$ and are ranked based on their performance.
